Wandercode: An Interaction Design for Code Recommenders to Reduce Information Overload, Ease Exploration, and Save Screen Space

In this paper, we present Wandercode, a novel interaction design for recommender systems that recommend code locations to aid programmers in software development tasks. In particular, our design aims to improve upon prior designs by reducing information overload, by better supporting the exploration of recommendations, and by making more efficient use of screen space. During our design process, we developed a set of design dimensions to aid others in the design of code recommenders. To validate our design, we implemented a prototype of our design as an Atom code editor extension with support for the Java programming language, and conducted an empirical user evaluation comparing our graph-based Wandercode design to a control design representative of prior list-based interaction designs for code recommenders. The results showed that, compared with the control design, Wandercode helped participants complete tasks more quickly, reduced their cognitive load, and was viewed more favorably by participants.

==> sec-acknowledgments.tex <==
%!TEX root = ./main.tex



% use section* for acknowledgement
\section*{Acknowledgments}

Anonymized. 

%This material is based upon work supported by Microsoft and the National Science Foundation (NSF) under Grant No.\ 1302117.
%
%Any opinions, findings, and conclusions or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of the NSF.

